Higher-order exchange interactions in two-dimensional magnets

Magnetism in recently discovered van der Waals materials has opened new avenues in the study of fundamental spin interactions in truly two-dimensions. A paramount question is what effect higher-order interactions beyond bilinear Heisenberg exchange have on the magnetic properties of few-atom thick compounds. Here we demonstrate that biquadratic exchange interactions, which is the simplest and most natural form of non-Heisenberg coupling, assume a key role in the magnetic properties of layered magnets. Using a combination of nonperturbative analytical techniques, non-collinear first-principles methods and classical Monte Carlo calculations that incorporate higher-order exchange, we show that several quantities including magnetic anisotropies, spin-wave gaps and topological spin-excitations are intrinsically renormalized leading to further thermal stability of the layers. We develop a spin Hamiltonian that also contains antisymmetric exchanges (e.g. Dzyaloshinskii-Moriya interactions) to successfully rationalize numerous observations currently under debate, such as the non-Ising character of several compounds despite a strong magnetic anisotropy, peculiarities of the magnon spectrum of 2D magnets, and the discrepancy between measured and calculated Curie temperatures. Our results lay the foundation of a universal higher-order exchange theory for novel 2D magnetic design strategies.

==> ref_bq.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Elton Santos at 2019-12-08 15:01:47 +0000 


%% Saved with string encoding Unicode (UTF-8) 



@article{Hammel19,
	Author = {Lee, I. and Utermohlen, F. G and Kyusung, Hwang and Daniel Weber and Chi Zhang and Johan van Tol and Joshua E. Goldberger and Nandini Trivedi and P. Chris Hammel},
	Date-Added = {2019-12-08 15:01:33 +0000},
	Date-Modified = {2019-12-08 15:01:33 +0000},
	Journal = {arXiv:1902.00077},
	Title = {Fundamental Spin Interactions Underlying the Magnetic Anisotropy in the Kitaev Ferromagnet CrI3}}

@article{Haastrup_2018,
	Abstract = {We introduce the Computational 2D Materials Database (C2DB), which organises a variety of structural, thermodynamic, elastic, electronic, magnetic, and optical properties of around 1500 two-dimensional materials distributed over more than 30 different crystal structures. Material properties are systematically calculated by state-of-the-art density functional theory and many-body perturbation theory ( and the Bethe--Salpeter equation for  ∼250 materials) following a semi-automated workflow for maximal consistency and transparency. The C2DB is fully open and can be browsed online (http://c2db.fysik.dtu.dk) or downloaded in its entirety. In this paper, we describe the workflow behind the database, present an overview of the properties and materials currently available, and explore trends and correlations in the data. Moreover, we identify a large number of new potentially synthesisable 2D materials with interesting properties targeting applications within spintronics, (opto-)electronics, and plasmonics. The C2DB offers a comprehensive and easily accessible overview of the rapidly expanding family of 2D materials and forms an ideal platform for computational modeling and design of new 2D materials and van der Waals heterostructures.},
	Author = {Sten Haastrup and Mikkel Strange and Mohnish Pandey and Thorsten Deilmann and Per S Schmidt and Nicki F Hinsche and Morten N Gjerding and Daniele Torelli and Peter M Larsen and Anders C Riis-Jensen and Jakob Gath and Karsten W Jacobsen and Jens J{\o}rgen Mortensen and Thomas Olsen and Kristian S Thygesen},
	Date-Added = {2019-12-06 12:21:22 +0000},
	Date-Modified = {2019-12-06 12:21:22 +0000},
	Doi = {10.1088/2053-1583/aacfc1},
	Journal = {2D Materials},
	Month = {sep},
	Number = {4},
	Pages = {042002},
	Publisher = {{IOP} Publishing},
	Title = {The Computational 2D Materials Database: high-throughput modeling and discovery of atomically thin crystals},
	Url = {https://doi.org/10.1088%2F2053-1583%2Faacfc1},
	Volume = {5},
	Year = 2018,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F2053-1583%2Faacfc1},
	Bdsk-Url-2 = {https://doi.org/10.1088/2053-1583/aacfc1}}

@article{Basov:2017aa,
	Abstract = {The past decade has witnessed an explosion in the field of quantum materials, headlined by the predictions and discoveries of novel Landau-symmetry-broken phases in correlated electron systems, topological phases in systems with strong spin--orbit coupling, and ultra-manipulable materials platforms based on two-dimensional van der Waals crystals. Discovering pathways to experimentally realize quantum phases of matter and exert control over their properties is a central goal of modern condensed-matter physics, which holds promise for a new generation of electronic/photonic devices with currently inaccessible and likely unimaginable functionalities. In this Review, we describe emerging strategies for selectively perturbing microscopic interaction parameters, which can be used to transform materials into a desired quantum state. Particular emphasis will be placed on recent successes to tailor electronic interaction parameters through the application of intense fields, impulsive electromagnetic stimulation, and nanostructuring or interface engineering. Together these approaches outline a potential roadmap to an era of quantum phenomena on demand.},
	Author = {Basov, D. N. and Averitt, R. D. and Hsieh, D.},
	Da = {2017/11/01},
	Date-Added = {2019-12-06 12:20:28 +0000},
	Date-Modified = {2019-12-06 12:20:28 +0000},
	Doi = {10.1038/nmat5017},
	Id = {Basov2017},
	Isbn = {1476-4660},
	Journal = {Nature Materials},
	Number = {11},
	Pages = {1077--1088},
	Title = {Towards properties on demand in quantum materials},
	Ty = {JOUR},
	Url = {https://doi.org/10.1038/nmat5017},
	Volume = {16},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1038/nmat5017}}

@article{Orbach64,
	Author = {Huang, Nai Li and Orbach, R.},
	Date-Added = {2019-11-29 11:32:35 +0000},
	Date-Modified = {2019-11-29 11:32:55 +0000},
	Doi = {10.1103/PhysRevLett.12.275},
	Issue = {11},
	Journal = {Phys. Rev. Lett.},
	Month = {Mar},
	Numpages = {0},
	Pages = {275--276},
	Publisher = {American Physical Society},
	Title = {Biquadratic Superexchange},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.12.275},
	Volume = {12},
	Year = {1964},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.12.275},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.12.275}}

@article{Basov17,
	Abstract = {The past decade has witnessed an explosion in the field of quantum materials, headlined by the predictions and discoveries of novel Landau-symmetry-broken phases in correlated electron systems, topological phases in systems with strong spin--orbit coupling, and ultra-manipulable materials platforms based on two-dimensional van der Waals crystals. Discovering pathways to experimentally realize quantum phases of matter and exert control over their properties is a central goal of modern condensed-matter physics, which holds promise for a new generation of electronic/photonic devices with currently inaccessible and likely unimaginable functionalities. In this Review, we describe emerging strategies for selectively perturbing microscopic interaction parameters, which can be used to transform materials into a desired quantum state. Particular emphasis will be placed on recent successes to tailor electronic interaction parameters through the application of intense fields, impulsive electromagnetic stimulation, and nanostructuring or interface engineering. Together these approaches outline a potential roadmap to an era of quantum phenomena on demand.},
	Author = {Basov, D. N. and Averitt, R. D. and Hsieh, D.},
	Da = {2017/11/01},
	Date-Added = {2019-11-23 19:29:14 +0000},
	Date-Modified = {2019-11-23 19:29:30 +0000},
	Doi = {10.1038/nmat5017},
	Id = {Basov2017},
	Isbn = {1476-4660},
	Journal = {Nature Materials},
	Number = {11},
	Pages = {1077--1088},
	Title = {Towards properties on demand in quantum materials},
	Ty = {JOUR},
	Url = {https://doi.org/10.1038/nmat5017},
	Volume = {16},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1038/nmat5017}}

@article{Katsnelson19,
	Author = {M. M. S. Barbeau and M. Eckstein and M. I. Katsnelson and J. H. Mentink},
	Date-Added = {2019-11-23 19:06:53 +0000},
	Date-Modified = {2019-11-23 19:07:10 +0000},
	Doi = {10.21468/SciPostPhys.6.3.027},
	Issue = {3},
	Journal = {SciPost Phys.},
	Pages = {27},
	Publisher = {SciPost},
	Title = {{Optical control of competing exchange interactions and coherent spin-charge coupling in two-orbital Mott insulators}},
	Url = {https://scipost.org/10.21468/SciPostPhys.6.3.027},
	Volume = {6},
	Year = {2019},
	Bdsk-Url-1 = {https://scipost.org/10.21468/SciPostPhys.6.3.027},
	Bdsk-Url-2 = {https://doi.org/10.21468/SciPostPhys.6.3.027}}

@article{Mahanti10,
	Author = {Hayden, L. X. and Kaplan, T. A. and Mahanti, S. D.},
	Date-Added = {2019-11-23 18:46:28 +0000},
	Date-Modified = {2019-11-23 18:46:43 +0000},
	Doi = {10.1103/PhysRevLett.105.047203},
	Issue = {4},
	Journal = {Phys. Rev. Lett.},
	Month = {Jul},
	Numpages = {4},
	Pages = {047203},
	Publisher = {American Physical Society},
	Title = {Frustrated Classical Heisenberg and $XY$ Models in Two Dimensions with Nearest-Neighbor Biquadratic Exchange: Exact Solution for the Ground-State Phase Diagram},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.105.047203},
	Volume = {105},
	Year = {2010},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.105.047203},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.105.047203}}

@article{Bader96,
	Author = {Fullerton, Eric E. and Bader, S. D.},
	Date-Added = {2019-11-21 19:05:29 +0000},
	Date-Modified = {2019-11-21 19:05:38 +0000},
	Doi = {10.1103/PhysRevB.53.5112},
	Issue = {9},
	Journal = {Phys. Rev. B},
	Month = {Mar},
	Numpages = {0},
	Pages = {5112--5115},
	Publisher = {American Physical Society},
	Title = {Temperature-dependent biquadratic coupling in antiferromagnetically coupled Fe/FeSi multilayers},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.53.5112},
	Volume = {53},
	Year = {1996},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.53.5112},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.53.5112}}

@article{Jonge00,
	Author = {Strijkers, G. J. and Kohlhepp, J. T. and Swagten, H. J. M. and de Jonge, W. J. M.},
	Date-Added = {2019-11-21 19:04:10 +0000},
	Date-Modified = {2019-11-21 19:04:35 +0000},
	Doi = {10.1103/PhysRevLett.84.1812},
	Issue = {8},
	Journal = {Phys. Rev. Lett.},
	Month = {Feb},
	Numpages = {0},
	Pages = {1812--1815},
	Publisher = {American Physical Society},
	Title = {Origin of Biquadratic Exchange in $\mathrm{Fe}/\mathrm{Si}/\mathrm{Fe}$},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.84.1812},
	Volume = {84},
	Year = {2000},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.84.1812},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.84.1812}}

@article{Ochoa16,
	Author = {Kim, Se Kwon and Ochoa, H\'ector and Zarzuela, Ricardo and Tserkovnyak, Yaroslav},
	Date-Added = {2019-11-21 12:47:53 +0000},
	Date-Modified = {2019-11-21 12:48:04 +0000},
	Doi = {10.1103/PhysRevLett.117.227201},
	Issue = {22},
	Journal = {Phys. Rev. Lett.},
	Month = {Nov},
	Numpages = {5},
	Pages = {227201},
	Publisher = {American Physical Society},
	Title = {Realization of the Haldane-Kane-Mele Model in a System of Localized Spins},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.117.227201},
	Volume = {117},
	Year = {2016},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.117.227201},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.117.227201}}

@article{unifiedBQ,
	Author = {Hu, Jiangping and Xu, Bao and Liu, Wuming and Hao, Ning-Ning and Wang, Yupeng},
	Date-Added = {2019-11-20 11:32:52 +0000},
	Date-Modified = {2019-11-20 11:33:07 +0000},
	Doi = {10.1103/PhysRevB.85.144403},
	Issue = {14},
	Journal = {Phys. Rev. B},
	Month = {Apr},
	Numpages = {12},
	Pages = {144403},
	Publisher = {American Physical Society},
	Title = {Unified minimum effective model of magnetic properties of iron-based superconductors},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.85.144403},
	Volume = {85},
	Year = {2012},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.85.144403},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.85.144403}}

@article{Mermin66,
	Author = {Mermin, N. D. and Wagner, H.},
	Date-Added = {2019-11-18 17:00:42 +0000},
	Date-Modified = {2019-11-18 17:00:53 +0000},
	Doi = {10.1103/PhysRevLett.17.1133},
	Issue = {22},
	Journal = {Phys. Rev. Lett.},
	Month = {Nov},
	Numpages = {0},
	Pages = {1133--1136},
	Publisher = {American Physical Society},
	Title = {Absence of Ferromagnetism or Antiferromagnetism in One- or Two-Dimensional Isotropic Heisenberg Models},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.17.1133},
	Volume = {17},
	Year = {1966},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.17.1133},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.17.1133}}

@article{Fisk01,
	Author = {Coldea, R. and Hayden, S. M. and Aeppli, G. and Perring, T. G. and Frost, C. D. and Mason, T. E. and Cheong, S.-W. and Fisk, Z.},
	Date-Added = {2019-11-18 11:32:48 +0000},
	Date-Modified = {2019-11-18 11:33:02 +0000},
	Doi = {10.1103/PhysRevLett.86.5377},
	Issue = {23},
	Journal = {Phys. Rev. Lett.},
	Month = {Jun},
	Numpages = {0},
	Pages = {5377--5380},
	Publisher = {American Physical Society},
	Title = {Spin Waves and Electronic Interactions in ${\mathrm{La}}_{2}{\mathrm{CuO}}_{4}$},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.86.5377},
	Volume = {86},
	Year = {2001},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.86.5377},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.86.5377}}

@article{Castets72,
	Author = {Nauciel-Bloch, M. and Sarma, G. and Castets, A.},
	Date-Added = {2019-11-18 11:26:52 +0000},
	Date-Modified = {2019-11-18 11:27:10 +0000},
	Doi = {10.1103/PhysRevB.5.4603},
	Issue = {11},
	Journal = {Phys. Rev. B},
	Month = {Jun},
	Numpages = {0},
	Pages = {4603--4609},
	Publisher = {American Physical Society},
	Title = {Spin-One Heisenberg Ferromagnet in the Presence of Biquadratic Exchange},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.5.4603},
	Volume = {5},
	Year = {1972},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.5.4603},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.5.4603}}

@article{Elliott69,
	Abstract = {Recent optical experiments have shown that the two-magnon spectra of antiferromagnets cannot be properly understood using simple non-interacting spin-wave theory. In these experiments two magnons are created close together in real space where they interact strongly to produce large observable effects. They therefore provide an excellent opportunity to study magnon-magnon interactions. A general theory of the two-magnon states using Green function methods is developed and the results applied to the spin-only antiferromagnet RbMnF3 and to CoF2 where the orbital contribution to the magnetic moment is important. The predicted optical properties are in good agreement with experiment.},
	Author = {R J Elliott and M F Thorpe},
	Date-Added = {2019-11-18 11:23:47 +0000},
	Date-Modified = {2019-11-18 11:23:56 +0000},
	Doi = {10.1088/0022-3719/2/9/312},
	Journal = {Journal of Physics C: Solid State Physics},
	Month = {sep},
	Number = {9},
	Pages = {1630--1643},
	Publisher = {{IOP} Publishing},
	Title = {The effects of magnon-magnon interaction on the two-magnon spectra of antiferromagnets},
	Url = {https://doi.org/10.1088%2F0022-3719%2F2%2F9%2F312},
	Volume = {2},
	Year = 1969,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F0022-3719%2F2%2F9%2F312},
	Bdsk-Url-2 = {https://doi.org/10.1088/0022-3719/2/9/312}}

@article{TingYu19,
	Annote = {doi: 10.1021/acs.nanolett.9b00553},
	Author = {Zhang, Zhaowei and Shang, Jingzhi and Jiang, Chongyun and Rasmita, Abdullah and Gao, Weibo and Yu, Ting},
	Booktitle = {Nano Letters},
	Da = {2019/05/08},
	Date = {2019/05/08},
	Date-Added = {2019-11-16 17:43:20 +0000},
	Date-Modified = {2019-11-16 17:43:33 +0000},
	Doi = {10.1021/acs.nanolett.9b00553},
	Isbn = {1530-6984},
	Journal = {Nano Letters},
	Journal1 = {Nano Lett.},
	M3 = {doi: 10.1021/acs.nanolett.9b00553},
	Month = {05},
	Number = {5},
	Pages = {3138--3142},
	Publisher = {American Chemical Society},
	Title = {Direct Photoluminescence Probing of Ferromagnetism in Monolayer Two-Dimensional CrBr3},
	Ty = {JOUR},
	Url = {https://doi.org/10.1021/acs.nanolett.9b00553},
	Volume = {19},
	Year = {2019},
	Year1 = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1021/acs.nanolett.9b00553}}

@article{kostya19,
	Abstract = {The study of atomically thin ferromagnetic crystals has led to the discovery of unusual magnetic behaviour and provided insight into the magnetic properties of bulk materials. However, the experimental techniques that have been used to explore ferromagnetism in such materials cannot probe the magnetic field directly. Here, we show that ballistic Hall micromagnetometry can be used to measure the magnetization of individual two-dimensional ferromagnets. Our devices are made by van der Waals assembly in such a way that the investigated ferromagnetic crystal is placed on top of a multi-terminal Hall bar made from encapsulated graphene. We use the micromagnetometry technique to study atomically thin chromium tribromide (CrBr3). We find that the material remains ferromagnetic down to monolayer thickness and exhibits strong out-of-plane anisotropy. We also find that the magnetic response of CrBr3 varies little with the number of layers and its temperature dependence cannot be described by the simple Ising model of two-dimensional ferromagnetism.},
	Author = {Kim, M. and Kumaravadivel, P. and Birkbeck, J. and Kuang, W. and Xu, S. G. and Hopkinson, D. G. and Knolle, J. and McClarty, P. A. and Berdyugin, A. I. and Ben Shalom, M. and Gorbachev, R. V. and Haigh, S. J. and Liu, S. and Edgar, J. H. and Novoselov, K. S. and Grigorieva, I. V. and Geim, A. K.},
	Da = {2019/10/01},
	Date-Added = {2019-11-16 17:40:57 +0000},
	Date-Modified = {2019-11-16 17:41:32 +0000},
	Doi = {10.1038/s41928-019-0302-6},
	Id = {Kim2019},
	Isbn = {2520-1131},
	Journal = {Nature Electronics},
	Number = {10},
	Pages = {457--463},
	Title = {Micromagnetometry of two-dimensional ferromagnets},
	Ty = {JOUR},
	Url = {https://doi.org/10.1038/s41928-019-0302-6},
	Volume = {2},
	Year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1038/s41928-019-0302-6}}

@article{Mak19,
	Abstract = {Two-dimensional magnetic semiconductors such as CrI3 are a new class of van der Waals material that may allow for the development of novel 2D spintronic devices. While strong magnetic anisotropy within the CrI3 layers stabilizes ferromagnetism down to a monolayer, weak antiferromagnetic coupling between the layers gives rise to extremely large tunnel magnetoresistance. We use a combination of tunneling and magneto-optical measurements to investigate the entire 2D chromium trihalide family (CrX3, X = I, Br, Cl). Our results elucidate both the interlayer coupling and intralayer spin Hamiltonian for all three materials, and further demonstrate that ferromagnetism can be stabilized in monolayer CrBr3 and bilayer CrCl3 without strong anisotropy.We conduct a comprehensive study of three different magnetic semiconductors, CrI3, CrBr3, and CrCl3, by incorporating both few-layer and bilayer samples in van der Waals tunnel junctions. We find that the interlayer magnetic ordering, exchange gap, magnetic anisotropy, and magnon excitations evolve systematically with changing halogen atom. By fitting to a spin wave theory that accounts for nearest-neighbor exchange interactions, we are able to further determine a simple spin Hamiltonian describing all three systems. These results extend the 2D magnetism platform to Ising, Heisenberg, and XY spin classes in a single material family. Using magneto-optical measurements, we additionally demonstrate that ferromagnetism can be stabilized down to monolayer in more isotropic CrBr3, with transition temperature still close to that of the bulk.},
	Author = {Kim, Hyun Ho and Yang, Bowen and Li, Siwen and Jiang, Shengwei and Jin, Chenhao and Tao, Zui and Nichols, George and Sfigakis, Francois and Zhong, Shazhou and Li, Chenghe and Tian, Shangjie and Cory, David G. and Miao, Guo-Xing and Shan, Jie and Mak, Kin Fai and Lei, Hechang and Sun, Kai and Zhao, Liuyan and Tsen, Adam W.},
	Date-Added = {2019-11-16 17:38:37 +0000},
	Date-Modified = {2019-11-16 17:38:49 +0000},
	Doi = {10.1073/pnas.1902100116},
	Eprint = {https://www.pnas.org/content/116/23/11131.full.pdf},
	Issn = {0027-8424},
	Journal = {Proceedings of the National Academy of Sciences},
	Number = {23},
	Pages = {11131--11136},
	Publisher = {National Academy of Sciences},
	Title = {Evolution of interlayer and intralayer magnetism in three atomically thin chromium trihalides},
	Url = {https://www.pnas.org/content/116/23/11131},
	Volume = {116},
	Year = {2019},
	Bdsk-Url-1 = {https://www.pnas.org/content/116/23/11131},
	Bdsk-Url-2 = {https://doi.org/10.1073/pnas.1902100116}}

@article{Dyson56,
	Author = {Dyson, Freeman J.},
	Date-Added = {2019-11-14 15:56:25 +0000},
	Date-Modified = {2019-11-14 15:56:35 +0000},
	Doi = {10.1103/PhysRev.102.1217},
	Issue = {5},
	Journal = {Phys. Rev.},
	Month = {Jun},
	Numpages = {0},
	Pages = {1217--1230},
	Publisher = {American Physical Society},
	Title = {General Theory of Spin-Wave Interactions},
	Url = {https://link.aps.org/doi/10.1103/PhysRev.102.1217},
	Volume = {102},
	Year = {1956},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRev.102.1217},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRev.102.1217}}

@book{Baxter16,
	Author = {Rodney J. Baxter},
	Date-Added = {2019-11-11 11:08:25 +0000},
	Date-Modified = {2019-11-11 11:09:07 +0000},
	Publisher = {Elsevier},
	Title = {Exactly Solved Models in Statistical Mechanics},
	Year = {2016}}

@incollection{ANDERSON63,
	Abstract = {Publisher Summary
This chapter discusses that the subject of exchange in magnetic materials is divided into two parts, referring to insulators and to metals. This distinction is useful from the magnetic point of view because in insulators the spins and magnetic moments whose alignments lead to magnetic effects are certainly localizable so that phenomenologically is described by a spin Hamiltonian that contains spin operators and exchange terms of Heisenberg type. It discusses that there is relationship among the mechanisms important in metals, such as conduction electron polarization, and those in insulators. The chapter provides historical discussion of the subjects of antiferromagnetism and of exchange in insulators. It focuses on the Heisenberg Hamiltonian, with a brief derivation and a discussion of some of the statistical theories of magnetism based upon it, primarily molecular field theory, which is by far the most generally useful in the experimental measurement of exchange. The chapter also describes older theories and presents ideas about super-exchange, and gives a discussion and a diagrammatic classification of all the possible higher-order processes.},
	Author = {Philip W. Anderson},
	Date-Added = {2019-11-09 17:49:42 +0000},
	Date-Modified = {2019-11-09 17:49:56 +0000},
	Doi = {https://doi.org/10.1016/S0081-1947(08)60260-X},
	Editor = {Frederick Seitz and David Turnbull},
	Issn = {0081-1947},
	Pages = {99 - 214},
	Publisher = {Academic Press},
	Series = {Solid State Physics},
	Title = {Theory of Magnetic Exchange Interactions:Exchange in Insulators and Semiconductors},
	Url = {http://www.sciencedirect.com/science/article/pii/S008119470860260X},
	Volume = {14},
	Year = {1963},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S008119470860260X},
	Bdsk-Url-2 = {https://doi.org/10.1016/S0081-1947(08)60260-X}}

@article{Takahashi77,
	Abstract = {The ground-state energy E and momentum distribution nk of the electrons are expanded from the atomic limit for the half-filled Hubbard model. The coefficients of expansion are represented by the spin correlation functions of the spin 1/2 Heisenberg model. Using the spin-wave theory, approximate values of coefficients are calculated for the square lattice and the simple cubic lattice. In one dimension, the theory shows a good agreement with the exact solution. An effective spin Hamiltonian for the half-filled Hubbard model with arbitrary hopping integrals is obtained up to the fifth order. It is shown that the fourth term contains four spin interactions.},
	Author = {M Takahashi},
	Date-Added = {2019-11-09 15:02:22 +0000},
	Date-Modified = {2019-11-09 15:02:30 +0000},
	Doi = {10.1088/0022-3719/10/8/031},
	Journal = {Journal of Physics C: Solid State Physics},
	Month = {apr},
	Number = {8},
	Pages = {1289--7301},
	Publisher = {{IOP} Publishing},
	Title = {Half-filled Hubbard model at low temperature},
	Url = {https://doi.org/10.1088%2F0022-3719%2F10%2F8%2F031},
	Volume = {10},
	Year = 1977,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F0022-3719%2F10%2F8%2F031},
	Bdsk-Url-2 = {https://doi.org/10.1088/0022-3719/10/8/031}}

@book{Dionne-book,
	Author = {Gerald F. Dionne},
	Date-Added = {2019-11-09 14:39:08 +0000},
	Date-Modified = {2019-11-09 14:40:17 +0000},
	Publisher = {Springer, Boston, MA},
	Title = {Magnetic Oxides},
	Year = {2009}}

@article{Kitaev06,
	Abstract = {A spin-1/2 system on a honeycomb lattice is studied. The interactions between nearest neighbors are of XX, YY or ZZ type, depending on the direction of the link; different types of interactions may differ in strength. The model is solved exactly by a reduction to free fermions in a static Z2 gauge field. A phase diagram in the parameter space is obtained. One of the phases has an energy gap and carries excitations that are Abelian anyons. The other phase is gapless, but acquires a gap in the presence of magnetic field. In the latter case excitations are non-Abelian anyons whose braiding rules coincide with those of conformal blocks for the Ising model. We also consider a general theory of free fermions with a gapped spectrum, which is characterized by a spectral Chern number ν. The Abelian and non-Abelian phases of the original model correspond to ν=0 and ν=$\pm$1, respectively. The anyonic properties of excitation depend on ν mod 16, whereas ν itself governs edge thermal transport. The paper also provides mathematical background on anyons as well as an elementary theory of Chern number for quasidiagonal matrices.},
	Author = {Alexei Kitaev},
	Date-Added = {2019-11-08 12:01:13 +0000},
	Date-Modified = {2019-11-08 12:01:13 +0000},
	Doi = {https://doi.org/10.1016/j.aop.2005.10.005},
	Issn = {0003-4916},
	Journal = {Annals of Physics},
	Note = {January Special Issue},
	Number = {1},
	Pages = {2 - 111},
	Title = {Anyons in an exactly solved model and beyond},
	Url = {http://www.sciencedirect.com/science/article/pii/S0003491605002381},
	Volume = {321},
	Year = {2006},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0003491605002381},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.aop.2005.10.005}}

@article{Blugel01,
	Author = {Kurz, Ph. and Bihlmayer, G. and Hirai, K. and Bl\"ugel, S.},
	Date-Added = {2019-11-07 12:47:52 +0000},
	Date-Modified = {2019-11-07 12:48:14 +0000},
	Doi = {10.1103/PhysRevLett.86.1106},
	Issue = {6},
	Journal = {Phys. Rev. Lett.},
	Month = {Feb},
	Numpages = {0},
	Pages = {1106--1109},
	Publisher = {American Physical Society},
	Title = {Three-Dimensional Spin Structure on a Two-Dimensional Lattice: Mn $/$Cu(111)},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.86.1106},
	Volume = {86},
	Year = {2001},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.86.1106},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.86.1106}}

@article{Bozorth59,
	Author = {Bozorth, R.M. and Kramer, Vivian},
	Date-Added = {2019-11-05 14:33:52 +0000},
	Date-Modified = {2019-11-05 14:34:06 +0000},
	Doi = {10.1051/jphysrad:01959002002-3039300},
	Hal_Id = {jpa-00236056},
	Hal_Version = {v1},
	Journal = {{J. Phys. Radium}},
	Keywords = {chromium compounds ; cobalt compounds ; erbium compounds ; holmium compounds ; iron compounds ; lead compounds ; lithium compounds ; magnetism ; manganese compounds ; nickel compounds},
	Number = {2-3},
	Pages = {393-401},
	Pdf = {https://hal.archives-ouvertes.fr/jpa-00236056/file/ajp-jphysrad_1959_20_2-3_393_0.pdf},
	Title = {{Some ferrimagnetic and antiferromagnetic materials at low temperatures}},
	Url = {https://hal.archives-ouvertes.fr/jpa-00236056},
	Volume = {20},
	Year = {1959},
	Bdsk-Url-1 = {https://hal.archives-ouvertes.fr/jpa-00236056},
	Bdsk-Url-2 = {https://doi.org/10.1051/jphysrad:01959002002-3039300}}

@article{Corliss59,
	Author = {Hastings, J. M. and Elliott, N. and Corliss, L. M.},
	Date-Added = {2019-11-05 12:51:43 +0000},
	Date-Modified = {2019-11-05 12:51:57 +0000},
	Doi = {10.1103/PhysRev.115.13},
	Issue = {1},
	Journal = {Phys. Rev.},
	Month = {Jul},
	Numpages = {0},
	Pages = {13--17},
	Publisher = {American Physical Society},
	Title = {Antiferromagnetic Structures of Mn${\mathrm{S}}_{2}$, Mn${\mathrm{Se}}_{2}$, and Mn${\mathrm{Te}}_{2}$},
	Url = {https://link.aps.org/doi/10.1103/PhysRev.115.13},
	Volume = {115},
	Year = {1959},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRev.115.13},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRev.115.13}}

@article{Makimura93,
	Abstract = {Raman spectra of the two-dimensional antiferromagnet MnPSe3 are measured in the temperature region between 18 and 297 K. Below TN=74+or-2 K an anomalous enhancement of some Raman-active phonon peaks is observed. A new phonon peak appears below TN at 86 cm-1. The relation between its behaviour and the magnetic ordering as explained in terms of the spin-dependent phonon Raman process. A peak at 133 cm-1 (T=18 K) shifts to low frequency with increasing temperature and disappears above TN. It is assigned to a one-magnon Raman peak.},
	Author = {C Makimura and T Sekine and Y Tanokura and K Kurosawa},
	Date-Added = {2019-11-05 12:48:12 +0000},
	Date-Modified = {2019-11-05 12:48:24 +0000},
	Doi = {10.1088/0953-8984/5/5/013},
	Journal = {Journal of Physics: Condensed Matter},
	Month = {feb},
	Number = {5},
	Pages = {623--632},
	Publisher = {{IOP} Publishing},
	Title = {Raman scattering in the two-dimensional antiferromagnet {MnPSe}3},
	Url = {https://doi.org/10.1088%2F0953-8984%2F5%2F5%2F013},
	Volume = {5},
	Year = 1993,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F0953-8984%2F5%2F5%2F013},
	Bdsk-Url-2 = {https://doi.org/10.1088/0953-8984/5/5/013}}

@article{Kim2019,
	Abstract = {Magnetic ordering in the two-dimensional (2D) limit has been one of the most important issues in condensed matter physics for the past few decades. The recent discovery of new magnetic van der Waals materials heralds a much-needed easy route for the studies of 2D magnetism: the thickness dependence of the magnetic ordering has been examined using Ising- and XXZ-type magnetic van der Waals materials. Here, we investigated the magnetic ordering of MnPS3, a 2D antiferromagnetic material of the Heisenberg-type, by Raman spectroscopy from bulk all the way down to the bilayer. The phonon modes that involve the vibrations of Mn ions exhibit characteristic changes as the temperature gets lowered through the N{\'e}el temperature. In bulk MnPS3, the Raman peak at ~155 cm−1 becomes considerably broadened near the N{\'e}el temperature, and upon further cooling is subsequently red-shifted. The measured peak positions and polarization dependences of the Raman spectra are in excellent agreement with our first-principles calculations. In few-layer MnPS3, the peak at ~155 cm−1 exhibits the characteristic red-shift at low temperatures down to the bilayer, indicating that the magnetic ordering is surprisingly stable at such a thin limit. Our work sheds light on the hitherto unexplored magnetic ordering in the Heisenberg-type antiferromagnetic systems in the atomic-layer limit.},
	Author = {Kangwon Kim and Soo Yeon Lim and Jungcheol Kim and Jae-Ung Lee and Sungmin Lee and Pilkwang Kim and Kisoo Park and Suhan Son and Cheol-Hwan Park and Je-Geun Park and Hyeonsik Cheong},
	Date-Added = {2019-11-05 12:44:53 +0000},
	Date-Modified = {2019-11-05 12:45:06 +0000},
	Doi = {10.1088/2053-1583/ab27d5},
	Journal = {2D Materials},
	Month = {jul},
	Number = {4},
	Pages = {041001},
	Publisher = {{IOP} Publishing},
	Title = {Antiferromagnetic ordering in van der Waals 2D magnetic material {MnPS}3 probed by Raman spectroscopy},
	Url = {https://doi.org/10.1088%2F2053-1583%2Fab27d5},
	Volume = {6},
	Year = 2019,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F2053-1583%2Fab27d5},
	Bdsk-Url-2 = {https://doi.org/10.1088/2053-1583/ab27d5}}

@article{Novoselov19,
	Abstract = {The family of two-dimensional (2D) materials grows day by day, hugely expanding the scope of possible phenomena to be explored in two dimensions, as well as the possible van der Waals (vdW) heterostructures that one can create. Such 2D materials currently cover a vast range of properties. Until recently, this family has been missing one crucial member: 2D magnets. The situation has changed over the past 2 years with the introduction of a variety of atomically thin magnetic crystals. Here we will discuss the difference between magnetic states in 2D materials and in bulk crystals and present an overview of the 2D magnets that have been explored recently. We will focus on the case of the two most studied systems---semiconducting CrI3 and metallic Fe3GeTe2---and illustrate the physical phenomena that have been observed. Special attention will be given to the range of new van der Waals heterostructures that became possible with the appearance of 2D magnets, offering new perspectives in this rapidly expanding field.},
	Author = {Gibertini, M. and Koperski, M. and Morpurgo, A. F. and Novoselov, K. S.},
	Da = {2019/05/01},
	Date-Added = {2019-09-18 19:28:06 +0100},
	Date-Modified = {2019-09-18 19:28:26 +0100},
	Doi = {10.1038/s41565-019-0438-6},
	Id = {Gibertini2019},
	Isbn = {1748-3395},
	Journal = {Nature Nanotechnology},
	Number = {5},
	Pages = {408--419},
	Title = {Magnetic 2D materials and heterostructures},
	Ty = {JOUR},
	Url = {https://doi.org/10.1038/s41565-019-0438-6},
	Volume = {14},
	Year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1038/s41565-019-0438-6}}

@article{Gongeaav4450,
	Abstract = {The alignment of the magnetic properties of atoms gives rise to a wealth of simple and exotic properties that can be exploited. As the dimension of the material is reduced, such that the atoms are in a single monolayer, it was widely believed that thermal fluctuations overwhelm and prevent magnetic ordering. Gong and Zhang review the developments that have followed the recent discovery of magnetism in two-dimensional materials. Recognizing that magnetic anisotropy can be used to induce stable magnetism in atomic monolayers, they provide an overview of the materials available and the physical understanding of the effects and then discuss how these effects could be exploited for widespread practical applications.Science, this issue p. eaav4450BACKGROUNDThe electron can be considered as a tiny magnet, with two opposite poles defining its magnetic field associated with the spin and orbital motion. When such minuscule magnets are collectively aligned as a result of the inherent coupling, ferromagnetism emerges. However, ferromagnetism had long been believed to hardly survive in two-dimensional (2D) systems because of the enhanced thermal fluctuations revealed by the Mermin-Wagner theorem. The recent discovery of 2D magnetic crystals showed that magnetic anisotropy could stabilize the long-range magnetic order by opening up an excitation gap to resist the thermal agitation. Two-dimensional magnetic crystals constitute ideal platforms to experimentally access the fundamental physics of magnetism in reduced dimensions. In contrast to the traditional magnetic thin films, 2D materials largely decouple from the substrates, allow electrical control, are mechanically flexible, and are open to chemical functionalization. These attributes make 2D magnets accessible, engineerable, and integrable into emergent heterostructures for previously unachieved properties and applications such as atomically thin magneto-optical and magnetoelectric devices for ultracompact spintronics, on-chip optical communications, and quantum computing.ADVANCESMagnetism has been explored in 2D materials for more than a decade. Magnetic moments have been created through defect engineering based on vacancies, adatoms, boundaries, and edges; band structure engineering, assisted by density functional theory calculations, has raised possibilities of 2D magnetism in, for instance, gated bilayer graphene and doped GaSe; the proximity effect has been applied to imprint spin polarization in 2D materials from magnetic substrates. However, these prior efforts centered on extrinsically induced magnetic response.In early 2017, the first observations of long-range magnetic order in pristine 2D crystals were reported in Cr2Ge2Te6 and CrI3. Both are magnetic insulators, yet with distinct magnetic properties. In contrast, 2D Fe3GeTe2 was recently proven to be a magnetic conductor. Itinerant magnets and magnetic insulators possess diverse application perspectives. Molecular beam epitaxial growth of 2D magnets has been reported for Fe3GeTe2, VSe2, MnSex, and Cr2Ge2Te6. The typical Curie temperatures of 2D magnets are much lower than those of their 3D counterparts. However, this does not fundamentally exclude the possibility of high-temperature 2D magnets. Efforts toward this goal have shown promise.When van der Waals (vdW) magnets contact nonmagnetic materials, time reversal asymmetry could be introduced in the original nonmagnets, likely leading to, for example, valley polarization in transition metal dichalcogenides or quantum anomalous Hall states in topological insulators. However, it should be noted that 2D magnets{\textquoteright} properties are susceptible to the contacting materials. Stacking vdW magnets with dissimilar materials could enrich the landscape of emergent phenomena by causing, for example, heterostructure multiferroicity, unconventional superconductivity, and the quantum anomalous Hall effect.Two-dimensional spintronic and magnonic devices have begun to emerge. Spin-orbit torque has been generated while spin-polarized current is injected from 2D materials (e.g., WTe2) into magnetic substrates; conversely, a spin wave has been pumped from magnetic substrates into 2D materials for spin-charge conversion. Magnetic tunnel junctions with 2D magnets (e.g., CrI3) as tunneling barriers exhibit giant tunneling magnetoresistance at low temperatures. New concepts of spin field-effect transistors based on 2D magnets have been reported as well.OUTLOOKMost currently available 2D magnets rely on mechanical exfoliation and only work at low temperatures. The wafer-scale synthesis of 2D magnets that operate above room temperature is a prerequisite for the development of practical applications. In the longer run, the monolithic integration of such 2D magnets with other functional materials is crucial for practical scalability. Spintronic devices require efficient electrical modulation of 2D magnets, long-distance transport of spins or spin waves, and efficient tunneling and injection of spins at various junctions. The practical development of low-power spintronic devices needs to be compatible with the existing complementary metal-oxide semiconductor technology (e.g., impedance match and affordable power supply). Furthermore, the exotic spin textures, quantum phases, and quasiparticles in 2D magnetic crystals and hetero-interfaces could lead to new ways of computation and communication. We envision that successive breakthroughs in 2D magnets could usher in a new era of information technologies with exciting applications in computing, sensing, and data storage.Two-dimensional magnetic crystals: The atomically thin crystalline hosts of magneto-optic and magnetoelectric effects.2D magnetic crystals, including 2D ferromagnets (left) and 2D antiferromagnets with diverse intra- and interplane magnetic configurations (right), can exhibit a plethora of magneto-optic and magnetoelectric effects. The red and blue protrusions in the atomic Lego depict the opposite local spins in magnetic layers.Magnetism, originating from the moving charges and spin of elementary particles, has revolutionized important technologies such as data storage and biomedical imaging, and continues to bring forth new phenomena in emergent materials and reduced dimensions. The recently discovered two-dimensional (2D) magnetic van der Waals crystals provide ideal platforms for understanding 2D magnetism, the control of which has been fueling opportunities for atomically thin, flexible magneto-optic and magnetoelectric devices (such as magnetoresistive memories and spin field-effect transistors). The seamless integration of 2D magnets with dissimilar electronic and photonic materials opens up exciting possibilities for unprecedented properties and functionalities. We review the progress in this area and identify the possible directions for device applications, which may lead to advances in spintronics, sensors, and computing.},
	Author = {Gong, Cheng and Zhang, Xiang},
	Date-Added = {2019-09-18 19:25:44 +0100},
	Date-Modified = {2019-09-18 19:25:44 +0100},
	Doi = {10.1126/science.aav4450},
	Elocation-Id = {eaav4450},
	Eprint = {https://science.sciencemag.org/content/363/6428/eaav4450.full.pdf},
	Issn = {0036-8075},
	Journal = {Science},
	Number = {6428},
	Publisher = {American Association for the Advancement of Science},
	Title = {Two-dimensional magnetic crystals and emergent heterostructure devices},
	Url = {https://science.sciencemag.org/content/363/6428/eaav4450},
	Volume = {363},
	Year = {2019},
	Bdsk-Url-1 = {https://science.sciencemag.org/content/363/6428/eaav4450},
	Bdsk-Url-2 = {https://doi.org/10.1126/science.aav4450}}

@article{Cava19,
	Author = {Kong, Tai and Guo, Shu and Ni, Danrui and Cava, Robert J.},
	Date-Added = {2019-09-18 19:15:51 +0100},
	Date-Modified = {2019-09-18 19:16:00 +0100},
	Doi = {10.1103/PhysRevMaterials.3.084419},
	Issue = {8},
	Journal = {Phys. Rev. Materials},
	Month = {Aug},
	Numpages = {5},
	Pages = {084419},
	Publisher = {American Physical Society},
	Title = {Crystal structure and magnetic properties of the layered van der Waals compound $\mathrm{VB}{\mathrm{r}}_{3}$},
	Url = {https://link.aps.org/doi/10.1103/PhysRevMaterials.3.084419},
	Volume = {3},
	Year = {2019},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevMaterials.3.084419},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevMaterials.3.084419}}

@article{VI3_19,
	Author = {Tian, Shangjie and Zhang, Jian-Feng and Li, Chenghe and Ying, Tianping and Li, Shiyan and Zhang, Xiao and Liu, Kai and Lei, Hechang},
	Date-Added = {2019-09-18 19:12:22 +0100},
	Date-Modified = {2019-09-18 19:12:38 +0100},
	Doi = {10.1021/jacs.8b13584},
	Eprint = {https://doi.org/10.1021/jacs.8b13584},
	Journal = {Journal of the American Chemical Society},
	Note = {PMID: 30856325},
	Number = {13},
	Pages = {5326-5333},
	Title = {Ferromagnetic van der Waals Crystal VI3},
	Url = {https://doi.org/10.1021/jacs.8b13584},
	Volume = {141},
	Year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1021/jacs.8b13584}}

@article{Nagaev_1982,
	Abstract = {This review is primarily devoted to a discussion of isotropic magnetic materials with localized magnetic
moments between which the exchange interaction is more complex than in the usual Heisenberg model. They include insulators for which the biquadratic or multispin exchange mechanisms are comparable with the bilinear exchange, conductors which do not satisfy the conditions of validity of the RKKY indirect exchange theory, and the nuclear magnetic material solid helium. Additionally, an analysis is made of high-anisotropy magnetic materials behaving similarly to isotropic non-Heisenberg materials. These anisotropic materials have anomalous properties, compared with the Heisenberg case. Experimental data on these materials and their theoretical interpretation are given. The following topics are discussed: 1) the conditions for a strong non-Heisenberg exchange and non-Heisenberg Hamiltonians; 2) quadrupole ordering and order-proper disorder phase transitions; 3) order-order and order-improper disorder phase transitions; 4) metamagnetism of isotropic materials; 5) normal sequences and "devil's ladders" of phase transitions between commensurable
structures; 6) canted antiferromagnetism of high-symmetry crystals which do not obey the condition for the existence of relativistic Dzyaloshinski{\~\i}-type interactions.},
	Author = {{\'{E}} L Nagaev},
	Date-Added = {2019-09-18 19:03:46 +0100},
	Date-Modified = {2019-09-18 19:03:46 +0100},
	Doi = {10.1070/pu1982v025n01abeh004495},
	Journal = {Soviet Physics Uspekhi},
	Month = {jan},
	Number = {1},
	Pages = {31--57},
	Publisher = {{IOP} Publishing},
	Title = {Anomalous magnetic structures and phase transitions in non-Heisenberg magnetic materials},
	Url = {https://doi.org/10.1070%2Fpu1982v025n01abeh004495},
	Volume = {25},
	Year = 1982,
	Bdsk-Url-1 = {https://doi.org/10.1070%2Fpu1982v025n01abeh004495},
	Bdsk-Url-2 = {https://doi.org/10.1070/pu1982v025n01abeh004495}}

@article{Ashvin09,
	Author = {Turner, Ari M. and Wang, Fa and Vishwanath, Ashvin},
	Date-Added = {2019-09-18 17:41:24 +0100},
	Date-Modified = {2019-09-18 17:41:35 +0100},
	Doi = {10.1103/PhysRevB.80.224504},
	Issue = {22},
	Journal = {Phys. Rev. B},
	Month = {Dec},
	Numpages = {9},
	Pages = {224504},
	Publisher = {American Physical Society},
	Title = {Kinetic magnetism and orbital order in iron telluride},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.80.224504},
	Volume = {80},
	Year = {2009},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.80.224504},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.80.224504}}

@article{Iron-BQ,
	Author = {Zhu, Hai-Feng and Cao, Hai-Yuan and Xie, Yun and Hou, Yu-Sheng and Chen, Shiyou and Xiang, Hongjun and Gong, Xin-Gao},
	Date-Added = {2019-09-18 17:39:22 +0100},
	Date-Modified = {2019-09-18 17:39:33 +0100},
	Doi = {10.1103/PhysRevB.93.024511},
	Issue = {2},
	Journal = {Phys. Rev. B},
	Month = {Jan},
	Numpages = {6},
	Pages = {024511},
	Publisher = {American Physical Society},
	Title = {Giant biquadratic interaction-induced magnetic anisotropy in the iron-based superconductor ${A}_{x}\mathrm{F}{\mathrm{e}}_{2\ensuremath{-}y}\mathrm{S}{\mathrm{e}}_{2}$},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.93.024511},
	Volume = {93},
	Year = {2016},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.93.024511},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.93.024511}}

@article{Kun98,
	Author = {Bhatt,R. N. and Yang,Kun},
	Date-Added = {2019-09-18 17:12:17 +0100},
	Date-Modified = {2019-09-18 17:12:26 +0100},
	Doi = {10.1063/1.367612},
	Eprint = {https://doi.org/10.1063/1.367612},
	Journal = {Journal of Applied Physics},
	Number = {11},
	Pages = {7231-7233},
	Title = {Non-Heisenberg couplings and ferromagnetic instability in a random antiferromagnetic spin-1 chain},
	Url = {https://doi.org/10.1063/1.367612},
	Volume = {83},
	Year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.1063/1.367612}}

@article{Bode07,
	Author = {Bode, M. and Heide, M. and von Bergmann, K. and Ferriani, P. and Heinze, S. and Bihlmayer, G. and Kubetzka, A. and Pietzsch, O. and Bl{\"u}gel, S. and Wiesendanger, R.},
	Date = {2007/05/10/online},
	Date-Added = {2019-07-11 21:48:17 +0200},
	Date-Modified = {2019-07-11 21:48:17 +0200},
	Day = {10},
	Journal = {Nature},
	L3 = {10.1038/nature05802;},
	Month = {05},
	Pages = {190 EP -},
	Publisher = {Nature Publishing Group SN -},
	Title = {Chiral magnetic order at surfaces driven by inversion asymmetry},
	Ty = {JOUR},
	Url = {https://doi.org/10.1038/nature05802},
	Volume = {447},
	Year = {2007},
	Bdsk-Url-1 = {https://doi.org/10.1038/nature05802}}

@article{Harris63,
	Author = {Harris, E. A. and Owen, J.},
	Date-Added = {2019-07-11 21:32:31 +0200},
	Date-Modified = {2019-07-11 21:32:41 +0200},
	Doi = {10.1103/PhysRevLett.11.9},
	Issue = {1},
	Journal = {Phys. Rev. Lett.},
	Month = {Jul},
	Numpages = {0},
	Pages = {9--10},
	Publisher = {American Physical Society},
	Title = {Biquadratic Exchange Between ${\mathrm{Mn}}^{2+}$ Ions in MgO},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.11.9},
	Volume = {11},
	Year = {1963},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.11.9},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.11.9}}

@article{Slonczewski91,
	Author = {Slonczewski, J. C.},
	Date-Added = {2019-07-11 21:04:19 +0200},
	Date-Modified = {2019-07-11 21:04:25 +0200},
	Doi = {10.1103/PhysRevLett.67.3172},
	Issue = {22},
	Journal = {Phys. Rev. Lett.},
	Month = {Nov},
	Numpages = {0},
	Pages = {3172--3175},
	Publisher = {American Physical Society},
	Title = {Fluctuation mechanism for biquadratic exchange coupling in magnetic multilayers},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.67.3172},
	Volume = {67},
	Year = {1991},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.67.3172},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.67.3172}}

@article{Wysocki:2011aa,
	Author = {Wysocki, Aleksander L. and Belashchenko, Kirill D. and Antropov, Vladimir P.},
	Date = {2011/03/06/online},
	Date-Added = {2019-07-11 20:28:07 +0200},
	Date-Modified = {2019-07-11 20:28:07 +0200},
	Day = {06},
	Journal = {Nature Physics},
	L3 = {10.1038/nphys1933;},
	M3 = {Article},
	Month = {03},
	Pages = {485 EP -},
	Publisher = {Nature Publishing Group SN -},
	Title = {Consistent model of magnetism in ferropnictides},
	Ty = {JOUR},
	Url = {https://doi.org/10.1038/nphys1933},
	Volume = {7},
	Year = {2011},
	Bdsk-Url-1 = {https://doi.org/10.1038/nphys1933}}

@article{Nicola15,
	Author = {Fedorova, Natalya S. and Ederer, Claude and Spaldin, Nicola A. and Scaramucci, Andrea},
	Date-Added = {2019-07-11 20:23:50 +0200},
	Date-Modified = {2019-07-11 20:24:00 +0200},
	Doi = {10.1103/PhysRevB.91.165122},
	Issue = {16},
	Journal = {Phys. Rev. B},
	Month = {Apr},
	Numpages = {14},
	Pages = {165122},
	Publisher = {American Physical Society},
	Title = {Biquadratic and ring exchange interactions in orthorhombic perovskite manganites},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.91.165122},
	Volume = {91},
	Year = {2015},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.91.165122},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.91.165122}}

@article{Slonczewski93,
	Author = {Slonczewski,J. C.},
	Date-Added = {2019-07-10 12:49:51 +0200},
	Date-Modified = {2019-07-10 12:50:01 +0200},
	Doi = {10.1063/1.353483},
	Eprint = {https://doi.org/10.1063/1.353483},
	Journal = {Journal of Applied Physics},
	Number = {10},
	Pages = {5957-5962},
	Title = {Origin of biquadratic exchange in magnetic multilayers (invited)},
	Url = {https://doi.org/10.1063/1.353483},
	Volume = {73},
	Year = {1993},
	Bdsk-Url-1 = {https://doi.org/10.1063/1.353483}}

@article{Demokritov98,
	Abstract = {An unusual interlayer coupling, recently discovered in layered magnetic systems, is analysed from the experimental and theoretical points of view. This coupling favours the  orientation of the magnetization of the adjacent magnetic films. It can be phenomenologically described by a term in the energy expression, which is biquadratic with respect to the magnetizations of the two films. The main experimental findings, as well as the theoretical models, explaining the phenomenon are discussed.},
	Author = {S O Demokritov},
	Date-Added = {2019-07-10 12:48:17 +0200},
	Date-Modified = {2019-07-10 12:48:28 +0200},
	Doi = {10.1088/0022-3727/31/8/003},
	Journal = {Journal of Physics D: Applied Physics},
	Month = {apr},
	Number = {8},
	Pages = {925--941},
	Publisher = {{IOP} Publishing},
	Title = {Biquadratic interlayer coupling in layered magnetic systems},
	Url = {https://doi.org/10.1088%2F0022-3727%2F31%2F8%2F003},
	Volume = {31},
	Year = 1998,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F0022-3727%2F31%2F8%2F003},
	Bdsk-Url-2 = {https://doi.org/10.1088/0022-3727/31/8/003}}

@book{deJonghbook,
	Author = {L.J. de Jongh},
	Date-Added = {2019-07-09 21:20:15 +0200},
	Date-Modified = {2019-07-09 21:20:15 +0200},
	Publisher = {Springer},
	Title = {Magnetic Properties of Layered Transition Metal Compounds},
	Year = {2012}}

@article{Guguchiaeaat3672,
	Abstract = {Transition metal dichalcogenides (TMDs) are interesting for understanding the fundamental physics of two-dimensional (2D) materials as well as for applications to many emerging technologies, including spin electronics. Here, we report the discovery of long-range magnetic order below TM = 40 and 100 K in bulk semiconducting TMDs 2H-MoTe2 and 2H-MoSe2, respectively, by means of muon spin rotation (μSR), scanning tunneling microscopy (STM), and density functional theory (DFT) calculations. The μSR measurements show the presence of large and homogeneous internal magnetic fields at low temperatures in both compounds indicative of long-range magnetic order. DFT calculations show that this magnetism is promoted by the presence of defects in the crystal. The STM measurements show that the vast majority of defects in these materials are metal vacancies and chalcogen-metal antisites, which are randomly distributed in the lattice at the subpercent level. DFT indicates that the antisite defects are magnetic with a magnetic moment in the range of 0.9 to 2.8 μB. Further, we find that the magnetic order stabilized in 2H-MoTe2 and 2H-MoSe2 is highly sensitive to hydrostatic pressure. These observations establish 2H-MoTe2 and 2H-MoSe2 as a new class of magnetic semiconductors and open a path to studying the interplay of 2D physics and magnetism in these interesting semiconductors.},
	Author = {Guguchia, Z. and Kerelsky, A. and Edelberg, D. and Banerjee, S. and von Rohr, F. and Scullion, D. and Augustin, M. and Scully, M. and Rhodes, D. A. and Shermadini, Z. and Luetkens, H. and Shengelaya, A. and Baines, C. and Morenzoni, E. and Amato, A. and Hone, J. C. and Khasanov, R. and Billinge, S. J. L. and Santos, E. and Pasupathy, A. N. and Uemura, Y. J.},
	Date-Added = {2019-07-09 21:16:36 +0200},
	Date-Modified = {2019-07-09 21:16:36 +0200},
	Doi = {10.1126/sciadv.aat3672},
	Elocation-Id = {eaat3672},
	Eprint = {https://advances.sciencemag.org/content/4/12/eaat3672.full.pdf},
	Journal = {Science Advances},
	Number = {12},
	Publisher = {American Association for the Advancement of Science},
	Title = {Magnetism in semiconducting molybdenum dichalcogenides},
	Url = {https://advances.sciencemag.org/content/4/12/eaat3672},
	Volume = {4},
	Year = {2018},
	Bdsk-Url-1 = {https://advances.sciencemag.org/content/4/12/eaat3672},
	Bdsk-Url-2 = {https://doi.org/10.1126/sciadv.aat3672}}

@article{CrI3_magnons_expermnt,
	Author = {Chen, Lebing and Chung, Jae-Ho and Gao, Bin and Chen, Tong and Stone, Matthew B. and Kolesnikov, Alexander I. and Huang, Qingzhen and Dai, Pengcheng},
	Doi = {10.1103/PhysRevX.8.041028},
	Issue = {4},
	Journal = {Phys. Rev. X},
	Month = {Nov},
	Numpages = {7},
	Pages = {041028},
	Publisher = {American Physical Society},
	Title = {Topological Spin Excitations in Honeycomb Ferromagnet ${\mathrm{CrI}}_{3}$},
	Url = {https://link.aps.org/doi/10.1103/PhysRevX.8.041028},
	Volume = {8},
	Year = {2018},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevX.8.041028},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevX.8.041028}}

@article{RuCl3,
	Author = {Plumb, K. W. and Clancy, J. P. and Sandilands, L. J. and Shankar, V. Vijay and Hu, Y. F. and Burch, K. S. and Kee, Hae-Young and Kim, Young-June},
	Doi = {10.1103/PhysRevB.90.041112},
	Issue = {4},
	Journal = {Phys. Rev. B},
	Month = {Jul},
	Numpages = {5},
	Pages = {041112},
	Publisher = {American Physical Society},
	Title = {$\ensuremath{\alpha}\ensuremath{-}{\mathrm{RuCl}}_{3}$: A spin-orbit assisted Mott insulator on a honeycomb lattice},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.90.041112},
	Volume = {90},
	Year = {2014},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.90.041112},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.90.041112}}

@article{RuCl3_2,
	Author = {Banerjee, A. and Bridges, C. A. and Yan, J.-Q. and Aczel, A. A. and Li, L. and Stone, M. B. and Granroth, G. E. and Lumsden, M. D. and Yiu, Y. and Knolle, J. and Bhattacharjee, S. and Kovrizhin, D. L. and Moessner, R. and Tennant, D. A. and Mandrus, D. G. and Nagler, S. E.},
	Day = {04},
	Journal = {Nature Materials},
	Month = {Apr},
	Note = {Article},
	Pages = {733 EP -},
	Publisher = {Nature Publishing Group SN -},
	Title = {Proximate Kitaev quantum spin liquid behaviour in a honeycomb magnet},
	Url = {https://doi.org/10.1038/nmat4604},
	Volume = {15},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1038/nmat4604}}

@article{Fe3GeTe2,
	Author = {Deng, Yujun and Yu, Yijun and Song, Yichen and Zhang, Jingzhao and Wang, Nai Zhou and Sun, Zeyuan and Yi, Yangfan and Wu, Yi Zheng and Wu, Shiwei and Zhu, Junyi},
	Journal = {Nature},
	Number = {7729},
	Pages = {94},
	Publisher = {Nature Publishing Group},
	Title = {Gate-tunable room-temperature ferromagnetism in two-dimensional Fe 3 GeTe 2},
	Volume = {563},
	Year = {2018}}

@article{2LCrI3,
	Author = {Jiang, Shengwei and Shan, Jie and Mak, Kin Fai},
	Journal = {Nature materials},
	Pages = {1},
	Publisher = {Nature Publishing Group},
	Title = {Electric-field switching of two-dimensional van der Waals magnets},
	Year = {2018}}

@article{2LCrI3_2,
	Author = {Wang, Zhe and Guti{\'e}rrez-Lezama, Ignacio and Ubrig, Nicolas and Kroner, Martin and Gibertini, Marco and Taniguchi, Takashi and Watanabe, Kenji and Imamo{\u{g}}lu, Ata{\c{c}} and Giannini, Enrico and Morpurgo, Alberto F},
	Journal = {Nature communications},
	Number = {1},
	Pages = {2516},
	Publisher = {Nature Publishing Group},
	Title = {Very large tunneling magnetoresistance in layered magnetic semiconductor CrI 3},
	Volume = {9},
	Year = {2018}}

@article{2LCrI3_3,
	Author = {Jiang, Peiheng and Li, Lei and Liao, Zhaoliang and Zhao, YX and Zhong, Zhicheng},
	Journal = {Nano letters},
	Number = {6},
	Pages = {3844--3849},
	Publisher = {ACS Publications},
	Title = {Spin Direction-Controlled Electronic Band Structure in Two-Dimensional Ferromagnetic CrI3},
	Volume = {18},
	Year = {2018}}

@article{2LCrI3_4,
	Author = {Farooq, M Umar and Hong, Jisang},
	Journal = {npj 2D Materials and Applications},
	Number = {1},
	Pages = {3},
	Publisher = {Nature Publishing Group},
	Title = {Switchable valley splitting by external electric field effect in graphene/CrI 3 heterostructures},
	Volume = {3},
	Year = {2019}}

@article{2LCrI3_5,
	Author = {Sivadas, Nikhil and Okamoto, Satoshi and Xu, Xiaodong and Fennie, Craig J and Xiao, Di},
	Journal = {Nano letters},
	Number = {12},
	Pages = {7658--7664},
	Publisher = {ACS Publications},
	Title = {Stacking-dependent magnetism in bilayer CrI3},
	Volume = {18},
	Year = {2018}}

@article{1LCrS2,
	Author = {Wang, Cong and Zhou, Xieyu and Pan, Yuhao and Qiao, Jingsi and Kong, Xianghua and Kaun, Chao-Cheng and Ji, Wei},
	Doi = {10.1103/PhysRevB.97.245409},
	Issue = {24},
	Journal = {Phys. Rev. B},
	Month = {Jun},
	Numpages = {11},
	Pages = {245409},
	Publisher = {American Physical Society},
	Title = {Layer and doping tunable ferromagnetic order in two-dimensional $\mathrm{Cr}{\mathrm{S}}_{2}$ layers},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.97.245409},
	Volume = {97},
	Year = {2018},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.97.245409},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.97.245409}}

@article{Koch,
	Author = {Pavarini, Eva and Koch, Erik and Anders, Frithjof and Jarrell, Mark},
	Journal = {Reihe Modeling and Simulation},
	Title = {Correlated electrons: from models to materials},
	Volume = {2},
	Year = {2012}}

@article{MC,
	Author = {Asselin, Pierre and Evans, Richard Francis L and Barker, Joe and Chantrell, Roy W and Yanes, Rocio and Chubykalo-Fesenko, Oksana and Hinzke, Denise and Nowak, Ulrich},
	Journal = {Physical Review B},
	Number = {5},
	Pages = {054415},
	Publisher = {APS},
	Title = {Constrained Monte Carlo method and calculation of the temperature dependence of magnetic anisotropy},
	Volume = {82},
	Year = {2010}}

@article{Evans14,
	Author = {Evans, Richard FL and Fan, Weijia J and Chureemart, Phanwadee and Ostler, Thomas A and Ellis, Matthew OA and Chantrell, Roy W},
	Date-Modified = {2019-11-11 09:11:25 +0000},
	Journal = {Journal of Physics: Condensed Matter},
	Number = {10},
	Pages = {103202},
	Publisher = {IOP Publishing},
	Title = {Atomistic spin model simulations of magnetic nanomaterials},
	Volume = {26},
	Year = {2014}}

@article{cri3,
	Abstract = {The observation of ferromagnetic order in a monolayer of CrI 3 has been recently reported, with a Curie temperature of 45 K and off-plane easy axis. Here we study the origin of magnetic anisotropy, a necessary ingredient to have magnetic order in two dimensions, combining two levels of modeling, density functional calculations and spin model Hamiltonians. We find two different contributions to the magnetic anisotropy of the material, favoring off-plane magnetization and opening a gap in the spin wave spectrum. First, ferromagnetic super-exchange across the ≃90 degree Cr--I--Cr bonds, are anisotropic, due to the spin--orbit interaction of the ligand I atoms. Second, a much smaller contribution that comes from the single ion anisotropy of the S   =  3/2 Cr atom. Our results permit to establish the XXZ Hamiltonian, with a very small single ion anisotropy, as the adequate spin model for this system. Using spin wave theory we estimate the Curie temperature and we highlight the essential role played by the gap that magnetic anisotropy induces on the magnon spectrum.},
	Author = {J L Lado and J Fern{\'a}ndez-Rossier},
	Journal = {2D Materials},
	Number = {3},
	Pages = {035002},
	Title = {On the origin of magnetic anisotropy in two dimensional CrI 3},
	Url = {http://stacks.iop.org/2053-1583/4/i=3/a=035002},
	Volume = {4},
	Year = {2017},
	Bdsk-Url-1 = {http://stacks.iop.org/2053-1583/4/i=3/a=035002}}

@article{HSE06,
	Author = {Krukau, Aliaksandr V and Vydrov, Oleg A and Izmaylov, Artur F and Scuseria, Gustavo E},
	Journal = {The Journal of chemical physics},
	Number = {22},
	Pages = {224106},
	Publisher = {AIP},
	Title = {Influence of the exchange screening parameter on the performance of screened hybrid functionals},
	Volume = {125},
	Year = {2006}}

@article{CrX3_linearresponse,
	Author = {Liu, Junyi and Sun, Qiang and Kawazoe, Yoshiyuki and Jena, Puru},
	Journal = {Physical Chemistry Chemical Physics},
	Number = {13},
	Pages = {8777--8784},
	Publisher = {Royal Society of Chemistry},
	Title = {Exfoliating biocompatible ferromagnetic Cr-trihalide monolayers},
	Volume = {18},
	Year = {2016}}

@article{CrGeTe,
	Author = {Gong, Cheng and Li, Lin and Li, Zhenglu and Ji, Huiwen and Stern, Alex and Xia, Yang and Cao, Ting and Bao, Wei and Wang, Chenzhe and Wang, Yuan and Qiu, Z. Q. and Cava, R. J. and Louie, Steven G. and Xia, Jing and Zhang, Xiang},
	Day = {08},
	Issn = {0028-0836},
	Journal = {Nature},
	Month = {Jun},
	Note = {Letter},
	Number = {7657},
	Pages = {265-269},
	Publisher = {Macmillan Publishers Limited, part of Springer Nature. All rights reserved.},
	Title = {Discovery of intrinsic ferromagnetism in two-dimensional van der Waals crystals},
	Url = {http://dx.doi.org/10.1038/nature22060},
	Volume = {546},
	Year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature22060}}

@article{Iexc1,
	Author = {Cardias, R and Szilva, A and Bergman, A and Di Marco, I and Katsnelson, MI and Lichtenstein, AI and Nordstr{\"o}m, L and Klautau, AB and Eriksson, O and Kvashnin, YO},
	Journal = {Scientific Reports},
	Publisher = {Nature Publishing Group},
	Title = {The Bethe-Slater curve revisited; new insights from electronic structure theory},
	Volume = {7},
	Year = {2017}}

@article{Iexc2,
	Author = {Pajda, M. and Kudrnovsk\'y, J. and Turek, I. and Drchal, V. and Bruno, P.},
	Doi = {10.1103/PhysRevB.64.174402},
	Issue = {17},
	Journal = {Phys. Rev. B},
	Month = {Oct},
	Numpages = {9},
	Pages = {174402},
	Publisher = {American Physical Society},
	Title = {Ab initio},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.64.174402},
	Volume = {64},
	Year = {2001},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.64.174402},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.64.174402}}

@article{CrI3exp,
	Author = {McGuire, Michael A and Dixit, Hemant and Cooper, Valentino R and Sales, Brian C},
	Journal = {Chemistry of Materials},
	Number = {2},
	Pages = {612--620},
	Publisher = {ACS Publications},
	Title = {Coupling of crystal structure and magnetism in the layered, ferromagnetic insulator CrI3},
	Volume = {27},
	Year = {2015}}

@article{exchange1,
	Author = {Kulish, Vadym V and Huang, Wei},
	Journal = {Journal of Materials Chemistry C},
	Number = {34},
	Pages = {8734--8741},
	Publisher = {Royal Society of Chemistry},
	Title = {Single-layer metal halides MX 2 (X= Cl, Br, I): stability and tunable magnetism from first principles and Monte Carlo simulations},
	Volume = {5},
	Year = {2017}}

@article{exchange2,
	Author = {Zhang, Wei-Bing and Qu, Qian and Zhu, Peng and Lam, Chi-Hang},
	Journal = {Journal of Materials Chemistry C},
	Number = {48},
	Pages = {12457--12468},
	Publisher = {Royal Society of Chemistry},
	Title = {Robust intrinsic ferromagnetism and half semiconductivity in stable two-dimensional single-layer chromium trihalides},
	Volume = {3},
	Year = {2015}}

@article{exchange3,
	Author = {Wang, Hongbo and Fan, Fengren and Zhu, Shasha and Wu, Hua},
	Journal = {EPL (Europhysics Letters)},
	Number = {4},
	Pages = {47001},
	Publisher = {IOP Publishing},
	Title = {Doping enhanced ferromagnetism and induced half-metallicity in CrI3 monolayer},
	Volume = {114},
	Year = {2016}}

@article{goodwin,
	Author = {Goodwin, Leif},
	Journal = {Journal of Physics: Condensed Matter},
	Number = {22},
	Pages = {3869},
	Publisher = {IOP Publishing},
	Title = {A new tight binding parameterization for carbon},
	Volume = {3},
	Year = {1991}}

@article{elf,
	Author = {Becke, Axel D and Edgecombe, Kenneth E},
	Journal = {The Journal of chemical physics},
	Number = {9},
	Pages = {5397--5403},
	Publisher = {AIP},
	Title = {A simple measure of electron localization in atomic and molecular systems},
	Volume = {92},
	Year = {1990}}

@article{cri3_nn,
	Author = {Zheng, Fawei and Zhao, Jize and Liu, Zheng and Li, Menglei and Zhou, Mei and Zhang, Shengbai and Zhang, Ping},
	Journal = {arXiv preprint arXiv:1709.05472},
	Title = {Tunable spin states in two-dimensional magnet CrI3},
	Year = {2017}}

@article{Fe_BQ,
	Author = {Spi{\v{s}}{\'a}k, D and Hafner, J},
	Journal = {Journal of magnetism and magnetic materials},
	Number = {3},
	Pages = {257--268},
	Publisher = {Elsevier},
	Title = {Theory of bilinear and biquadratic effect ofexchange interactions in iron: Bulk and surface},
	Volume = {168},
	Year = {1997}}

@article{FeIrRh_BQ,
	Author = {Meyer, Sebastian and Dup{\'e}, Bertrand and Ferriani, Paolo and Heinze, Stefan},
	Journal = {Physical Review B},
	Number = {9},
	Pages = {094408},
	Publisher = {APS},
	Title = {Dzyaloshinskii-Moriya interaction at an antiferromagnetic interface: First-principles study of Fe/Ir bilayers on Rh (001)},
	Volume = {96},
	Year = {2017}}

@article{FeIr_BQ,
	Author = {De{\'a}k, A and Szunyogh, L and Ujfalussy, B},
	Journal = {Physical Review B},
	Number = {22},
	Pages = {224413},
	Publisher = {APS},
	Title = {Thickness-dependent magnetic structure of ultrathin Fe/Ir (001) films: From spin-spiral states toward ferromagnetic order},
	Volume = {84},
	Year = {2011}}

@article{Hub2Heis,
	Author = {Cleveland, Charles L and Medina A, Rodrigo},
	Journal = {American Journal of Physics},
	Number = {1},
	Pages = {44--46},
	Publisher = {AAPT},
	Title = {Obtaining a Heisenberg Hamiltonian from the Hubbard model},
	Volume = {44},
	Year = {1976}}

@article{magfield4Hub,
	Author = {Yang, C and Kocharian, AN and Chiang, YL},
	Journal = {Journal of Physics: Condensed Matter},
	Number = {33},
	Pages = {7433},
	Publisher = {IOP Publishing},
	Title = {Phase transitions and exact ground-state properties of the one-dimensional Hubbard model in a magnetic field},
	Volume = {12},
	Year = {2000}}

@article{magfield4Hub2,
	Author = {Kioussis, N and Kocharian, AN and Park, S},
	Journal = {Journal of magnetism and magnetic materials},
	Number = {181},
	Pages = {575--576},
	Publisher = {Citeseer},
	Title = {One-dimensional Hubbard model in the presence of magnetic field},
	Volume = {177},
	Year = {1998}}

@book{1DHubbard_book,
	Author = {Essler, Fabian H. L. and Frahm, Holger and G{\"o}hmann, Frank and Kl{\"u}mper, Andreas and Korepin, Vladimir E.},
	Doi = {10.1017/CBO9780511534843},
	Place = {Cambridge},
	Publisher = {Cambridge University Press},
	Title = {The One-Dimensional Hubbard Model},
	Year = {2005},
	Bdsk-Url-1 = {https://doi.org/10.1017/CBO9780511534843}}

@article{VASP1,
	Author = {Kresse, Georg and Furthm{\"u}ller, J{\"u}rgen},
	Journal = {Physical review B},
	Number = {16},
	Pages = {11169},
	Publisher = {APS},
	Title = {Efficient iterative schemes for ab initio total-energy calculations using a plane-wave basis set},
	Volume = {54},
	Year = {1996}}

@article{PBE,
	Author = {Perdew, John P. and Burke, Kieron and Ernzerhof, Matthias},
	Doi = {10.1103/PhysRevLett.77.3865},
	Issue = {18},
	Journal = {Phys. Rev. Lett.},
	Month = {Oct},
	Numpages = {0},
	Pages = {3865--3868},
	Publisher = {American Physical Society},
	Title = {Generalized Gradient Approximation Made Simple},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.77.3865},
	Volume = {77},
	Year = {1996},
	Bdsk-File-1 = {YnBsaXN0MDDSAQIDBFxyZWxhdGl2ZVBhdGhZYWxpYXNEYXRhXxAvLi4vLi4vLi4vLi4vLi4vRG93bmxvYWRzL1BoeXNSZXZCLjgwLjIyNDUwNC5iaWJPEQFqAAAAAAFqAAIAAAxNYWNpbnRvc2ggSEQAAAAAAAAAAAAAAAAAAAAAAAAAQkQAAf////8WUGh5c1JldkIuODAuMjI0NTA0LmJpYgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA/////wAAAAAAAAAAAAAAAAAFAAIAAAogY3UAAAAAAAAAAAAAAAAACURvd25sb2FkcwAAAgAwLzpVc2Vyczplc2FudG9zOkRvd25sb2FkczpQaHlzUmV2Qi44MC4yMjQ1MDQuYmliAA4ALgAWAFAAaAB5AHMAUgBlAHYAQgAuADgAMAAuADIAMgA0ADUAMAA0AC4AYgBpAGIADwAaAAwATQBhAGMAaQBuAHQAbwBzAGgAIABIAEQAEgAuVXNlcnMvZXNhbnRvcy9Eb3dubG9hZHMvUGh5c1JldkIuODAuMjI0NTA0LmJpYgATAAEvAAAVAAIADv//AAAACAANABoAJABWAAAAAAAAAgEAAAAAAAAABQAAAAAAAAAAAAAAAAAAAcQ=},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.77.3865},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.77.3865}}

@article{Krukau2006,
	Author = {Krukau, Aliaksandr V and Vydrov, Oleg A and Izmaylov, Artur F and Scuseria, Gustavo E},
	Journal = {The Journal of chemical physics},
	Number = {22},
	Pages = {224106},
	Publisher = {AIP},
	Title = {Influence of the exchange screening parameter on the performance of screened hybrid functionals},
	Volume = {125},
	Year = {2006}}

@article{Liecht,
	Author = {Liechtenstein, A. I. and Anisimov, V. I. and Zaanen, J.},
	Doi = {10.1103/PhysRevB.52.R5467},
	Issue = {8},
	Journal = {Phys. Rev. B},
	Month = {Aug},
	Numpages = {0},
	Pages = {R5467--R5470},
	Publisher = {American Physical Society},
	Title = {Density-functional theory and strong interactions: Orbital ordering in Mott-Hubbard insulators},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.52.R5467},
	Volume = {52},
	Year = {1995},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.52.R5467},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.52.R5467}}

@article{Dudarev,
	Author = {Dudarev, S. L. and Botton, G. A. and Savrasov, S. Y. and Humphreys, C. J. and Sutton, A. P.},
	Doi = {10.1103/PhysRevB.57.1505},
	Issue = {3},
	Journal = {Phys. Rev. B},
	Month = {Jan},
	Numpages = {0},
	Pages = {1505--1509},
	Publisher = {American Physical Society},
	Title = {Electron-energy-loss spectra and the structural stability of nickel oxide: An LSDA+U study},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.57.1505},
	Volume = {57},
	Year = {1998},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.57.1505},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.57.1505}}

@article{rpa,
	Author = {Olsen, Thomas},
	Journal = {Physical Review B},
	Number = {12},
	Pages = {125143},
	Publisher = {APS},
	Title = {Assessing the performance of the random phase approximation for exchange and superexchange coupling constants in magnetic crystalline solids},
	Volume = {96},
	Year = {2017}}

@article{vs2,
	Author = {Zhuang, Houlong L and Hennig, Richard G},
	Journal = {Physical Review B},
	Number = {5},
	Pages = {054429},
	Publisher = {APS},
	Title = {Stability and magnetism of strongly correlated single-layer VS_2},
	Volume = {93},
	Year = {2016}}

@article{firstCrI3,
	Author = {Huang, Bevin and Clark, Genevieve and Navarro-Moratalla, Efr{\'e}n and Klein, Dahlia R. and Cheng, Ran and Seyler, Kyle L. and Zhong, Ding and Schmidgall, Emma and McGuire, Michael A. and Cobden, David H. and Yao, Wang and Xiao, Di and Jarillo-Herrero, Pablo and Xu, Xiaodong},
	Day = {07},
	Journal = {Nature},
	Month = {Jun},
	Pages = {270 EP -},
	Publisher = {Macmillan Publishers Limited, part of Springer Nature. All rights reserved. SN -},
	Title = {Layer-dependent ferromagnetism in a van der Waals crystal down to the monolayer limit},
	Url = {https://doi.org/10.1038/nature22391},
	Volume = {546},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1038/nature22391}}

@article{BQin3Dmagnets,
	Author = {Iwashita, Takashi and Ury{\^u}, Norikiyo},
	Journal = {Physical Review B},
	Number = {7},
	Pages = {3090},
	Publisher = {APS},
	Title = {Effects of biquadratic exchange in ferromagnets},
	Volume = {14},
	Year = {1976}}

@article{linrespU,
	Author = {Liu, Junyi and Sun, Qiang and Kawazoe, Yoshiyuki and Jena, Puru},
	Journal = {Physical Chemistry Chemical Physics},
	Number = {13},
	Pages = {8777--8784},
	Publisher = {Royal Society of Chemistry},
	Title = {Exfoliating biocompatible ferromagnetic Cr-trihalide monolayers},
	Volume = {18},
	Year = {2016}}

@article{oxidationU,
	Author = {Wang, Lei and Maxisch, Thomas and Ceder, Gerbrand},
	Journal = {Physical Review B},
	Number = {19},
	Pages = {195107},
	Publisher = {APS},
	Title = {Oxidation energies of transition metal oxides within the GGA+ U framework},
	Volume = {73},
	Year = {2006}}

@article{DMFTtrichalcogenides,
	Author = {Kim, Heung-Sik and Vanderbilt, David and Haule, Kristjan},
	Journal = {arXiv preprint arXiv:1808.09263},
	Title = {Mott metal-insulator transitions in pressurized layered trichalcogenides},
	Year = {2018}}

@article{bader,
	Author = {Tang, W and Sanville, E and Henkelman, G},
	Journal = {Journal of Physics: Condensed Matter},
	Number = {8},
	Pages = {084204},
	Publisher = {IOP Publishing},
	Title = {A grid-based Bader analysis algorithm without lattice bias},
	Volume = {21},
	Year = {2009}}

@article{metalmetal,
	Author = {Girerd, Jean Jacques and Journaux, Yves and Kahn, Olivier},
	Journal = {Chemical Physics Letters},
	Number = {3},
	Pages = {534--538},
	Publisher = {Elsevier},
	Title = {Natural or orthogonalized magnetic orbitals: Two alternative ways to describe the exchange interaction},
	Volume = {82},
	Year = {1981}}

@article{ligandCrI3,
	Abstract = {Bulk chromium tri-iodide (CrI3) has long been known as a layered van der Waals ferromagnet1. However, its monolayer form was only recently isolated and confirmed to be a truly two-dimensional (2D) ferromagnet2, providing a new platform for investigating light-matter interactions and magneto-optical phenomena in the atomically thin limit. Here, we report spontaneous circularly polarized photoluminescence in monolayer CrI3 under linearly polarized excitation, with helicity determined by the monolayer magnetization direction. In contrast, the bilayer CrI3 photoluminescence exhibits vanishing circular polarization, supporting the recently uncovered anomalous antiferromagnetic interlayer coupling in CrI3 bilayers2. Distinct from the Wannier-Mott excitons that dominate the optical response in well-known 2D van der Waals semiconductors3, our absorption and layer-dependent photoluminescence measurements reveal the importance of ligand-field and charge-transfer transitions to the optoelectronic response of atomically thin CrI3. We attribute the photoluminescence to a parity-forbidden d-d transition characteristic of Cr3+ complexes, which displays broad linewidth due to strong vibronic coupling and thickness-independent peak energy due to its localized molecular orbital nature.},
	Author = {Seyler, Kyle L. and Zhong, Ding and Klein, Dahlia R. and Gao, Shiyuan and Zhang, Xiaoou and Huang, Bevin and Navarro-Moratalla, Efr{\'e}n and Yang, Li and Cobden, David H. and McGuire, Michael A. and Yao, Wang and Xiao, Di and Jarillo-Herrero, Pablo and Xu, Xiaodong},
	Doi = {10.1038/s41567-017-0006-7},
	Issn = {1745-2481},
	Journal = {Nature Physics},
	Number = {3},
	Pages = {277-281},
	Title = {Ligand-field helical luminescence in a 2D ferromagnetic insulator},
	Url = {https://doi.org/10.1038/s41567-017-0006-7},
	Volume = {14},
	Year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.1038/s41567-017-0006-7}}

@article{rubyCr3,
	Author = {Van der Ziel, JP},
	Journal = {Physical Review B},
	Number = {7},
	Pages = {2846},
	Publisher = {APS},
	Title = {Spectrum of first-nearest-neighbor Cr 3+ pairs in ruby},
	Volume = {9},
	Year = {1974}}

@article{spin_chain,
	Author = {Bhatt, RN and Yang, Kun},
	Journal = {Journal of applied physics},
	Number = {11},
	Pages = {7231--7233},
	Publisher = {AIP},
	Title = {Non-Heisenberg couplings and ferromagnetic instability in a random antiferromagnetic spin-1 chain},
	Volume = {83},
	Year = {1998}}

@article{spin_chain2,
	Author = {Mila, Frederic and Zhang, Fu-Chun},
	Journal = {The European Physical Journal B-Condensed Matter and Complex Systems},
	Number = {1},
	Pages = {7--10},
	Publisher = {Springer},
	Title = {On the origin of biquadratic exchange in spin 1 chains},
	Volume = {16},
	Year = {2000}}

@article{ligandtheory,
	Author = {Griffith, JS and Orgel, LE},
	Journal = {Quarterly Reviews, Chemical Society},
	Number = {4},
	Pages = {381--393},
	Publisher = {Royal Society of Chemistry},
	Title = {Ligand-field theory},
	Volume = {11},
	Year = {1957}}

@article{andersonsuperexchnage,
	Author = {Anderson, Philip W},
	Journal = {Physical Review},
	Number = {1},
	Pages = {2},
	Publisher = {APS},
	Title = {New approach to the theory of superexchange interactions},
	Volume = {115},
	Year = {1959}}

@article{bruno2Dferro,
	Author = {Bruno, Patrick},
	Journal = {Physical Review B},
	Number = {7},
	Pages = {6015},
	Publisher = {APS},
	Title = {Spin-wave theory of two-dimensional ferromagnets in the presence of dipolar interactions and magnetocrystalline anisotropy},
	Volume = {43},
	Year = {1991}}

@article{quadrupolarphase,
	Author = {L{\"a}uchli, Andreas and Mila, Fr{\'e}d{\'e}ric and Penc, Karlo},
	Journal = {Physical review letters},
	Number = {8},
	Pages = {087205},
	Publisher = {APS},
	Title = {Quadrupolar phases of the S= 1 bilinear-biquadratic Heisenberg model on the triangular lattice},
	Volume = {97},
	Year = {2006}}

@article{frustrated,
	Author = {Kaplan, TA},
	Journal = {Physical Review B},
	Number = {1},
	Pages = {012407},
	Publisher = {APS},
	Title = {Frustrated classical Heisenberg model in one dimension with nearest-neighbor biquadratic exchange: Exact solution for the ground-state phase diagram},
	Volume = {80},
	Year = {2009}}

@article{MottBQ,
	Author = {Tanaka, Katsuhiro and Yokoyama, Yuto and Hotta, Chisa},
	Journal = {Journal of the Physical Society of Japan},
	Number = {2},
	Pages = {023702},
	Publisher = {The Physical Society of Japan},
	Title = {Origin of Biquadratic Exchange Interactions in a Mott Insulator as a Driving Force of Spin Nematic Order},
	Volume = {87},
	Year = {2018}}

@article{ligandBQ,
	Author = {Noodleman, Louis and Davidson, Ernest R},
	Journal = {Chemical physics},
	Number = {1},
	Pages = {131--143},
	Publisher = {Elsevier},
	Title = {Ligand spin polarization and antiferromagnetic coupling in transition metal dimers},
	Volume = {109},
	Year = {1986}}

@article{bulk_CrBr3,
	Author = {Alyoshin, VA and Berezin, VA and Tulin, VA},
	Journal = {Physical Review B},
	Number = {2},
	Pages = {719},
	Publisher = {APS},
	Title = {rf susceptibility of single-crystal CrBr 3 near the Curie temperature},
	Volume = {56},
	Year = {1997}}

@article{2LCrCl3,
	Author = {Cai, Xinghan and Song, Tiancheng and Wilson, Nathan P. and Clark, Genevieve and He, Minhao and Zhang, Xiaoou and Taniguchi, Takashi and Watanabe, Kenji and Yao, Wang and Xiao, Di and McGuire, Michael A. and Cobden, David H. and Xu, Xiaodong},
	Day = {12},
	Doi = {10.1021/acs.nanolett.9b01317},
	Issn = {1530-6984},
	Journal = {Nano Letters},
	Month = {Jun},
	Number = {6},
	Pages = {3993-3998},
	Publisher = {American Chemical Society},
	Title = {Atomically Thin CrCl3: An In-Plane Layered Antiferromagnetic Insulator},
	Url = {https://doi.org/10.1021/acs.nanolett.9b01317},
	Volume = {19},
	Year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1021/acs.nanolett.9b01317}}

@article{2D_database,
	Abstract = {Two-dimensional (2D) materials have emerged as promising candidates for next-generation electronic and optoelectronic applications. Yet, only a few dozen 2D materials have been successfully synthesized or exfoliated. Here, we search for 2D materials that can be easily exfoliated from their parent compounds. Starting from 108,423 unique, experimentally known 3D compounds, we identify a subset of 5,619 compounds that appear layered according to robust geometric and bonding criteria. High-throughput calculations using van der Waals density functional theory, validated against experimental structural data and calculated random phase approximation binding energies, further allowed the identification of 1,825 compounds that are either easily or potentially exfoliable. In particular, the subset of 1,036 easily exfoliable cases provides novel structural prototypes and simple ternary compounds as well as a large portfolio of materials to search from for optimal properties. For a subset of 258 compounds, we explore vibrational, electronic, magnetic and topological properties, identifying 56 ferromagnetic and antiferromagnetic systems, including half-metals and half-semiconductors.},
	Author = {Mounet, Nicolas and Gibertini, Marco and Schwaller, Philippe and Campi, Davide and Merkys, Andrius and Marrazzo, Antimo and Sohier, Thibault and Castelli, Ivano Eligio and Cepellotti, Andrea and Pizzi, Giovanni and Marzari, Nicola},
	Doi = {10.1038/s41565-017-0035-5},
	Issn = {1748-3395},
	Journal = {Nature Nanotechnology},
	Number = {3},
	Pages = {246-252},
	Title = {Two-dimensional materials from high-throughput computational exfoliation of experimentally known compounds},
	Url = {https://doi.org/10.1038/s41565-017-0035-5},
	Volume = {13},
	Year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.1038/s41565-017-0035-5}}

@article{Dvalue_bulk,
	Author = {Chen, Lebing and Chung, Jae-Ho and Gao, Bin and Chen, Tong and Stone, Matthew B and Kolesnikov, Alexander I and Huang, Qingzhen and Dai, Pengcheng},
	Journal = {arXiv preprint arXiv:1807.11452},
	Title = {Topological spin excitations in honeycomb ferromagnet CrI $ \_3$},
	Year = {2018}}

@article{Sorokin2017,
	Abstract = {The results of the work conducted by the institutes of the Far East Branch of the Russian Academy of Sciences (FEB RAS) to develop the IT infrastructure for solving general and specialized tasks for the benefit of scientists in the Far East of Russia are described. Approaches to resource management and regulations for their funding in the current legal functioning model of scientific organizations are presented.},
	Author = {Sorokin, A. A. and Makogonov, S. V. and Korolev, S. P.},
	Day = {01},
	Doi = {10.3103/S0147688217040153},
	Issn = {1934-8118},
	Journal = {Scientific and Technical Information Processing},
	Month = {Oct},
	Number = {4},
	Pages = {302--304},
	Title = {The Information Infrastructure for Collective Scientific Work in the Far East of Russia},
	Url = {https://doi.org/10.3103/S0147688217040153},
	Volume = {44},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.3103/S0147688217040153}}

@article{QE-2009,
	Author = {Paolo Giannozzi and Stefano Baroni and Nicola Bonini and Matteo Calandra and Roberto Car and Carlo Cavazzoni and Davide Ceresoli and Guido L Chiarotti and Matteo Cococcioni and Ismaila Dabo and Andrea {Dal Corso} and Stefano de Gironcoli and Stefano Fabris and Guido Fratesi and Ralph Gebauer and Uwe Gerstmann and Christos Gougoussis and Anton Kokalj and Michele Lazzeri and Layla Martin-Samos and Nicola Marzari and Francesco Mauri and Riccardo Mazzarello and Stefano Paolini and Alfredo Pasquarello and Lorenzo Paulatto and Carlo Sbraccia and Sandro Scandolo and Gabriele Sclauzero and Ari P Seitsonen and Alexander Smogunov and Paolo Umari and Renata M Wentzcovitch},
	Journal = {Journal of Physics: Condensed Matter},
	Number = {39},
	Pages = {395502 (19pp)},
	Title = {QUANTUM ESPRESSO: a modular and open-source software project for quantum simulations of materials},
	Url = {http://www.quantum-espresso.org},
	Volume = {21},
	Year = {2009},
	Bdsk-Url-1 = {http://www.quantum-espresso.org}}

@article{MP,
	Author = {Monkhorst, Hendrik J. and Pack, James D.},
	Doi = {10.1103/PhysRevB.13.5188},
	Issue = {12},
	Journal = {Phys. Rev. B},
	Month = {Jun},
	Numpages = {0},
	Pages = {5188--5192},
	Publisher = {American Physical Society},
	Title = {Special points for Brillouin-zone integrations},
	Url = {http://link.aps.org/doi/10.1103/PhysRevB.13.5188},
	Volume = {13},
	Year = {1976},
	Bdsk-Url-1 = {http://link.aps.org/doi/10.1103/PhysRevB.13.5188},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.13.5188}}

@article{MV,
	Author = {Marzari, Nicola and Vanderbilt, David and De Vita, Alessandro and Payne, M. C.},
	Doi = {10.1103/PhysRevLett.82.3296},
	Issue = {16},
	Journal = {Phys. Rev. Lett.},
	Month = {Apr},
	Numpages = {0},
	Pages = {3296--3299},
	Publisher = {American Physical Society},
	Title = {Thermal Contraction and Disordering of the Al(110) Surface},
	Url = {http://link.aps.org/doi/10.1103/PhysRevLett.82.3296},
	Volume = {82},
	Year = {1999},
	Bdsk-Url-1 = {http://link.aps.org/doi/10.1103/PhysRevLett.82.3296},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.82.3296}}

@article{lobster,
	Author = {Maintz, Stefan and Deringer, Volker L and Tchougr{\'e}eff, Andrei L and Dronskowski, Richard},
	Journal = {Journal of computational chemistry},
	Number = {11},
	Pages = {1030--1035},
	Publisher = {Wiley Online Library},
	Title = {LOBSTER: A tool to extract chemical bonding from plane-wave based DFT},
	Volume = {37},
	Year = {2016}}

@article{Alzate_Cardona_2019,
	Annote = {We present an adaptive algorithm for the optimal phase space sampling in Monte Carlo simulations of 3D Heisenberg spin systems. Based on a golden rule of the Metropolis algorithm which states that an acceptance rate of  is ideal to efficiently sample the phase space, the algorithm adaptively modifies a cone-based spin update method keeping the acceptance rate close to . We have assessed the efficiency of the adaptive algorithm through four different tests and contrasted its performance with that of other common spin update methods. In systems at low and high temperatures and anisotropies, the adaptive algorithm proved to be the most efficient for magnetization reversal and for the convergence to equilibrium of the thermal averages and the coercivity in hysteresis calculations. Thus, the adaptive algorithm can be used to significantly reduce the computational cost in Monte Carlo simulations of 3D Heisenberg spin systems.},
	Author = {J D Alzate-Cardona and D Sabogal-Su{\'{a}}rez and R F L Evans and E Restrepo-Parra},
	Doi = {10.1088/1361-648x/aaf852},
	Journal = {Journal of Physics: Condensed Matter},
	Month = {jan},
	Number = {9},
	Pages = {095802},
	Publisher = {{IOP} Publishing},
	Title = {Optimal phase space sampling for Monte Carlo simulations of Heisenberg spin systems},
	Url = {https://doi.org/10.1088%2F1361-648x%2Faaf852},
	Volume = {31},
	Year = 2019,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F1361-648x%2Faaf852},
	Bdsk-Url-2 = {https://doi.org/10.1088/1361-648x/aaf852}}

@article{Ellis,
	Author = {Ellis,M. O. A. and Evans,R. F. L. and Ostler,T. A. and Barker,J. and Atxitia,U. and Chubykalo-Fesenko,O. and Chantrell,R. W.},
	Doi = {10.1063/1.4930971},
	Eprint = {https://doi.org/10.1063/1.4930971},
	Journal = {Low Temperature Physics},
	Number = {9},
	Pages = {705-712},
	Title = {The Landau--Lifshitz equation in atomistic models},
	Url = {https://doi.org/10.1063/1.4930971},
	Volume = {41},
	Year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1063/1.4930971}}

@article{BQpictinides,
	Author = {Wysocki, Aleksander L and Belashchenko, Kirill D and Antropov, Vladimir P},
	Journal = {Nature Physics},
	Number = {6},
	Pages = {485},
	Publisher = {Nature Publishing Group},
	Title = {Consistent model of magnetism in ferropnictides},
	Volume = {7},
	Year = {2011}}

@article{FeN,
	Abstract = {Most of the experimentally discovered compounds in the iron--nitrogen system belong to the low concentration part of the Fe--N phase diagram. In our paper{,} which is based on ab initio calculations{,} we have studied the formation and stability of high-pressure iron mono-nitride phases{,} and in particular a new magnetic phase with a NiAs-type structure. We have investigated the role of dynamic{,} thermodynamic and electronic properties{,} such as electronic correlations and pressure-induced phase stabilisation. Additionally{,} we have demonstrated that the new hexagonal FeN phase is stable over a wide range of external pressures and can persist at zero pressure as a metastable phase. Further{,} we have shown that this phase has a relatively low Curie temperature and may possess non-collinear magnetism.},
	Author = {Kartsev, Alexey and Feya, Oleg D. and Bondarenko, Nina and Kvashnin, Alexander G.},
	Doi = {10.1039/C8CP07165A},
	Issue = {9},
	Journal = {Phys. Chem. Chem. Phys.},
	Pages = {5262-5273},
	Publisher = {The Royal Society of Chemistry},
	Title = {Stability and magnetism of FeN high-pressure phases},
	Url = {http://dx.doi.org/10.1039/C8CP07165A},
	Volume = {21},
	Year = {2019},
	Bdsk-Url-1 = {http://dx.doi.org/10.1039/C8CP07165A}}

@article{dmi-magnon,
	Author = {Kovalev, Alexey A. and Zyuzin, Vladimir A. and Li, Bo},
	Date-Modified = {2019-12-04 16:28:06 +0000},
	Doi = {10.1103/PhysRevB.95.165106},
	Issue = {16},
	Journal = {Phys. Rev. B},
	Month = {Apr},
	Numpages = {14},
	Pages = {165106},
	Publisher = {American Physical Society},
	Title = {Pumping of magnons in a Dzyaloshinskii-Moriya ferromagnet},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.95.165106},
	Volume = {95},
	Year = {2017},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.95.165106},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.95.165106}}

@article{Holstein40,
	Author = {Holstein, T. and Primakoff, H.},
	Date-Modified = {2019-11-14 16:06:17 +0000},
	Doi = {10.1103/PhysRev.58.1098},
	Issue = {12},
	Journal = {Phys. Rev.},
	Month = {Dec},
	Numpages = {0},
	Pages = {1098--1113},
	Publisher = {American Physical Society},
	Title = {Field Dependence of the Intrinsic Domain Magnetization of a Ferromagnet},
	Url = {https://link.aps.org/doi/10.1103/PhysRev.58.1098},
	Volume = {58},
	Year = {1940},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRev.58.1098},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRev.58.1098}}

@article{Owerre16,
	Author = {Owerre,S. A.},
	Date-Modified = {2019-11-21 12:44:45 +0000},
	Doi = {10.1063/1.4959815},
	Eprint = {https://doi.org/10.1063/1.4959815},
	Journal = {Journal of Applied Physics},
	Number = {4},
	Pages = {043903},
	Title = {Topological honeycomb magnon Hall effect: A calculation of thermal Hall conductivity of magnetic spin excitations},
	Url = {https://doi.org/10.1063/1.4959815},
	Volume = {120},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1063/1.4959815}}

@article{Haldane88,
	Author = {Haldane, F. D. M.},
	Date-Modified = {2019-11-21 11:09:59 +0000},
	Doi = {10.1103/PhysRevLett.61.2015},
	Issue = {18},
	Journal = {Phys. Rev. Lett.},
	Month = {Oct},
	Numpages = {0},
	Pages = {2015--2018},
	Publisher = {American Physical Society},
	Title = {Model for a Quantum Hall Effect without Landau Levels: Condensed-Matter Realization of the "Parity Anomaly"},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.61.2015},
	Volume = {61},
	Year = {1988},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.61.2015},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.61.2015}}

@article{Lado_2017,
	Abstract = {The observation of ferromagnetic order in a monolayer of CrI3 has been recently reported, with a Curie temperature of 45 K and off-plane easy axis. Here we study the origin of magnetic anisotropy, a necessary ingredient to have magnetic order in two dimensions, combining two levels of modeling, density functional calculations and spin model Hamiltonians. We find two different contributions to the magnetic anisotropy of the material, favoring off-plane magnetization and opening a gap in the spin wave spectrum. First, ferromagnetic super-exchange across the ≃90 degree Cr--I--Cr bonds, are anisotropic, due to the spin--orbit interaction of the ligand I atoms. Second, a much smaller contribution that comes from the single ion anisotropy of the S  =  3/2 Cr atom. Our results permit to establish the XXZ Hamiltonian, with a very small single ion anisotropy, as the adequate spin model for this system. Using spin wave theory we estimate the Curie temperature and we highlight the essential role played by the gap that magnetic anisotropy induces on the magnon spectrum.},
	Author = {J L Lado and J Fern{\'{a}}ndez-Rossier},
	Doi = {10.1088/2053-1583/aa75ed},
	Journal = {2D Materials},
	Month = {jun},
	Number = {3},
	Pages = {035002},
	Publisher = {{IOP} Publishing},
	Title = {On the origin of magnetic anisotropy in two dimensional {CrI}3},
	Url = {https://doi.org/10.1088%2F2053-1583%2Faa75ed},
	Volume = {4},
	Year = 2017,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F2053-1583%2Faa75ed},
	Bdsk-Url-2 = {https://doi.org/10.1088/2053-1583/aa75ed}}

@article{Rohart13,
	Author = {Rohart, S. and Thiaville, A.},
	Doi = {10.1103/PhysRevB.88.184422},
	Issue = {18},
	Journal = {Phys. Rev. B},
	Month = {Nov},
	Numpages = {8},
	Pages = {184422},
	Publisher = {American Physical Society},
	Title = {Skyrmion confinement in ultrathin film nanostructures in the presence of Dzyaloshinskii-Moriya interaction},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.88.184422},
	Volume = {88},
	Year = {2013},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.88.184422},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.88.184422}}

@article{Laurent18,
	Author = {Xu, Changsong and Feng, Junsheng and Xiang, Hongjun and Bellaiche, Laurent},
	Date-Modified = {2019-11-08 12:00:39 +0000},
	Journal = {npj Computational Materials},
	Number = {1},
	Pages = {57},
	Publisher = {Nature Publishing Group},
	Title = {Interplay between Kitaev interaction and single ion anisotropy in ferromagnetic CrI 3 and CrGeTe 3 monolayers},
	Volume = {4},
	Year = {2018}}

@article{kitaev_concept,
	Author = {Takagi, Hidenori and Takayama, Tomohiro and Jackeli, George and Khaliullin, Giniyat and Nagler, Stephen E},
	Journal = {Nature Reviews Physics},
	Pages = {1},
	Publisher = {Nature Publishing Group},
	Title = {Concept and realization of Kitaev quantum spin liquids},
	Year = {2019}}

